A Contrastive Knowledge Transfer Framework for Model Compression and Transfer Learning

Knowledge Transfer (KT) achieves competitive performance and is widely used for image classification tasks in model compression and transfer learning. Existing KT works transfer the information from a large model ("teacher") to train a small model ("student") by minimizing the difference of their conditionally independent output distributions. However, these works overlook the high-dimension structural knowledge from the intermediate representations of the teacher, which leads to limited effectiveness, and they are motivated by various heuristic intuitions, which makes it difficult to generalize. This paper proposes a novel Contrastive Knowledge Transfer Framework (CKTF), which enables the transfer of sufficient structural knowledge from the teacher to the student by optimizing multiple contrastive objectives across the intermediate representations between them. Also, CKTF provides a generalized agreement to existing KT techniques and increases their performance significantly by deriving them as specific cases of CKTF. The extensive evaluation shows that CKTF consistently outperforms the existing KT works by 0.04% to 11.59% in model compression and by 0.4% to 4.75% in transfer learning on various models and datasets.

==> related_works.tex <==
% !TEX root = main.tex
\section{Background and Related Works}\label{sec:related_works}

% Hinton et al.~\cite{hinton2015distilling} proposed the idea of Knowledge Transfer (KT) to improve the performance of the small, fast models by transferring the knowledge from the large, cumbersome models during training. Existing knowledge KT techniques can be broadly classified into three categories, including transferring hard logits, transferring soft logits, and transferring intermediate representations. Ba et al. proposed hard-logits-based KT technique~\cite{ba2014deep}, which minimizes squared difference (RMSE) between the logits (output of the last fully-connected layer) of the teacher and the softmax output of the shallow student. Hinton et al. introduced transferring soft logits~\cite{hinton2015distilling} where the student minimizes the sum of two objective functions: (1) cross entropy loss between the soft logits, and (2) cross entropy loss between the softmax output and correct labels of the dataset. Romero et al. proposed FitNet, which extended transferring soft logits by using not only the soft outputs but also the intermediate representations learned by the teacher~\cite{venkatesan2016diving}. Later, transferring FSP matrix~\cite{yim2017gift} and attention~\cite{zagoruyko2016paying} were proposed, which are also based on transferring the intermediate representations. More recently, other papers~\cite{ahn2019variational,huang2017like,kim2018paraphrasing,koratana2019lit} have also proposed various forms of computations based on the intermediate representations. 


% However, these KT methods lack the commonly agreed theory, and they achieve limited accuracy improvement compared to training the small model without KT. 




% The contrastive objective we use in this paper is the same as that used in CMC (Tian et al., 2019). But we derive from a different perspective and give a rigorous proof that our objective is a lower bound on mutual information. Our objective is also related to the InfoNCE and NCE objectives introduced in (Oord et al., 2018; Gutmann & Hyvärinen, 2010). Oord et al. (2018) use contrastive learning in the context of self-supervised representations learning. They show that their objective maximizes a lower bound on mutual information. 



\boldhdr{Knowledge Transfer}
%
Various Knowledge Transfer (KT) techniques have been investigated under Deep Neural Networks to improve the performance of the small, fast networks by transferring knowledge from the large, cumbersome networks during training.
%
Ba et al. proposed hard-logits-based KT technique~\cite{ba2014deep}, which minimizes \yt{the} squared difference (RMSE) between the logits (output of the last fully-connected layer) of the deep teacher and the softmax output of the shallow student. Recent work Contrastive Representation Distillation CRD\cite{} also transferred hard logits but from another perspective by applying NCE loss~\cite{}. Hinton et al. introduced transferring soft logits~\cite{hinton2015distilling} where the student minimizes the sum of two objective functions, including cross-entropy loss between the teacher's and student's soft logits (softmax outputs), and cross-entropy loss with the ground-truth labels of the dataset. 
%
Romero et al. proposed FitNet, which extended transferring soft logits by using not only the softmax outputs but also the intermediate representations learned by the teacher~\cite{venkatesan2016diving}. Later, transferring FSP matrix~\cite{yim2017gift} and attention~\cite{zagoruyko2016paying} were proposed, which are also based on transferring the intermediate representations. More recently, other papers~\cite{ahn2019variational,huang2017like,kim2018paraphrasing,koratana2019lit} also proposed various computations based on the intermediate representations. 
%
However, these various KT works are motivated by different intuitions and lack a commonly agreed theory. This makes it challenging to generalize and create new techniques more ethically. Also, none of the existing KT works significantly outperform transferring soft logits~\cite{} (termed conventional KD) for model compression and transfer learning tasks. 
%
This paper summarizes the existing KT methods as special cases of the proposed framework. More importantly, incorporating the existing works into the proposed framework enhances their performance.



% \smalskip
\boldhdr{Contrastive Learning}
%
Contrastive learning has achieved competitive performance in self-supervised representations learning~\cite{}. 
Contrastive losses-based models have outperformed other methods in a large margin~\cite{}. 
The contrastive learning objective is to maximize a lower bound on the mutual information between the different views of the data~\cite{}. 
Recently it has been extended to Transformer-based model compression and language understanding tasks~\cite{}. 
However, the effectiveness of contrastive learning on intermediate representations of image-classification models, serving for model compression and unsupervised transfer learning tasks, is currently unexplored. 
% However, the intermediate representations based contrastive learning for knowledge transfer in image classification has not been studied before, especially for both model compression and transfer learning tasks. 
% Different from prior work, we propose the use of contrastive objective for intermediate-representation based model compression and cross-domain transfer learning tasks.




% =============================== >
% Summarize the related works we compare as follows:
